Multiple-Environment Markov Decision Processes

We introduce Multi-Environment Markov Decision Processes (MEMDPs) which are MDPs with a set of probabilistic transition functions. The goal in a MEMDP is to synthesize a single controller with guaranteed performances against all environments even though the environment is unknown a priori. While MEMDPs can be seen as a special class of partially observable MDPs, we show that several verification problems that are undecidable for partially observable MDPs, are decidable for MEMDPs and sometimes have even efficient solutions.

==> conclusion.tex <==
\section{Conclusion}

Recap

Generalization: We can work with different reachability and safety objectives,
and also mix reachability and safety.
For reachability, safety, and mixed objectives, we can generalize the algorithms
to the $k$-environment case. For almost-sure and limit-sure problems, this will
incur an exponential in~$k$ only. Notice that such an exponential also appears
in multi-objective reachability in MDPs~\cite{EKVY-lmcs08}.

\paragraph{Future work} settling the exact complexity of the quantitative case.
Mean payoff and discounted sum ongoing work?


==> hardness.tex <==
\section{Hardness}
\label{section:hardness}

The following \textsf{Subset-Product} problem is NP-hard. Given positive integers $v_1,\ldots,v_n$
and $V = v_1v_2\ldots v_n$ encoded in binary, decide whether there exists a subset $I
\subseteq \{1,\ldots,n\}$ such that $\Pi_{i \in I} v_i = \sqrt{V}$.

We reduce this problem to quantitative reachability in MEMDPs:
\begin{theorem}
	Given an MEMDP~$M$, one target state~$T$, and $\alpha_1,\alpha_2 \in [0,1]$, it is NP-hard to decide
	whether there exists a strategy~$\sigma$ such that
	$\pr_{M_i,s_0}^\sigma[\objreach(T)] \geq \alpha_i$ for each~$i=1,2$.
\end{theorem}
%\begin{proof}
	We fix an instance of the problem, and construct the following MEMDP.
	\begin{figure}[h!]
		\begin{center}
			\begin{tikzpicture}
			\tikzstyle{every state}=[minimum size=3pt,inner sep=0pt,node distance=2cm]
			\tikzstyle{every node}=[font=\small]
			\node[state] at (0,0) (s1) {$s_1$};
			\node[below right of=s1,node distance=40pt] (s1q){};
			\node[state,right of=s1,node distance=3cm] (nop) {};
			\fill (s1q) circle(2pt);
			%\node[below right of=s1] (s1q) {} circ(2pt);
			\node[state,below of=s1] (s2) {$s_2$};
			\node[below right of=s2,node distance=40pt] (s2q){};
			\fill (s2q) circle(2pt);
			\node[state, below of=s2] (s3) {$s_3$};
			\node[below of=s3] (s4) {$\vdots$};
			\node[below right of=s4,node distance=20pt] (s4q){};
			\fill (s4q) circle(2pt);
			\node[state,below of=s3,accepting] (sn) {$s_n$};
			\path[draw,-latex'] 
			(s1) edge[bend left] node[right]{$a$} (s1q) 
			(s1q) edge[bend left] node[right]{$\frac{1}{v_1}$} (s2) 
			(s1q) edge[bend right] node[left]{$1-\frac{1}{v_1}$} (nop) 
			(s1) edge[bend right] node[left]{$b$} (s2) 
			(s2) edge[bend left] node[right]{$a$} (s2q)
			(s2q) edge[bend left] node[below]{$\frac{1}{v_2}$} (s3) 
			(s2q) edge[bend right] node[left]{$1-\frac{1}{v_2}$} (nop) 
			(s2) edge[bend right] node[left]{$b$} (s3)
			(s4) edge[bend left] node[right]{$a$} (s4q)
			(s4) edge[bend right] node[left]{$b$} (sn)
			(s4q) edge[bend right] node[left]{$1-\frac{1}{v_n}$} (nop)
			(s4q) edge[bend left] node[right]{$\frac{1}{v_n}$} (sn);
		\end{tikzpicture}
		\end{center}
	\end{figure}
	The figure depicts the MDP~$M_1$, while $M_2$ is obtained by inversing the roles
	of~$a$ and~$b$. We let~$s_n$ be the target state.
	Let us denote $W = 1/V$.
	We will prove that $M$ has a strategy achieving the probabilities
	$(\sqrt{W},\sqrt{W})$ for reaching~$s_n$ 
	if, and only if the \textsf{Subset-Product} problem has a solution.
	Notice that the reduction is polynomial since all probabilities can be encoded
	in polynomial time.

	Observe that each pure strategy~$\sigma$ corresponds
	a set $S_\sigma=\{ i \mid \sigma(s_i,b) = 1\}$.
	We have that $\pr_{M_2,s_1}^\sigma[\objreach(T)] = \prod_{i \in
	S_\sigma}\frac{1}{v_i}$, and
	$\pr_{M_1,s_1}^\sigma[\objreach(T)] = \prod_{i \not\in
	S_\sigma}\frac{1}{v_i}$
	%W\big(\prod_{i \in
	%S_\sigma}\frac{1}{v_i}\big)^{-1}$. 
	Therefore, a pure strategy with values 
	$(\sqrt{W},\sqrt{W})$ yields a solution to the \textsf{Subset-product} problem, and
	conversely. 
	To establish the reduction, we need to show that if some arbitrary strategy achieves the probability vector
	$(\sqrt{W},\sqrt{W})$ in~$M$, then there is a pure strategy achieving the same
	vector. 
	\medskip

	To ease reading, for any strategy~$\sigma$, let us denote $p^\sigma_i =
	\pr_{M_i,s_1}^\sigma[\objreach(T)]$.
	Note that strategies do not need memory on this MEMDP: any state~$s_i$ uniquely
	determines the history. We thus concentrate on randomized memoryless strategies. 
	Let $\Sigma^D$ denote the set of deterministic strategies.

	\textbf{Claim:} For any stationary strategy~$\sigma$, there exists
	$(\lambda_\pi)_{\pi \in \Sigma^D}$ with $0\leq \lambda_\pi \leq 1$
	and $\sum_{\pi\in \Sigma^D} \lambda_\pi = 1$ such that
	$p_i^\sigma = \sum_{\pi\in \Sigma^D}\lambda_\pi p^\pi_i$ for
	all~$i=1,2$.

	The claim can be proved as follows. There is a finite number of deterministic
	strategies, each corresponding to a word in $(a+b)^n$. By summing over all
	runs leading to~$s_n$, we write
	$p^\sigma_j = \sum_{\pi \in (a+b)^n} \prod_{i=1}^n \sigma(s_i,\pi_i)
	\delta_j(s_i,\pi_i,s_{i+1})$
	so we let $\lambda_\pi = \prod_{i=1}^n \sigma(s_i,\pi_i)$, 
	and observe that $\prod_{i=1}^n \delta_j(s_i,\pi_i,s_{i+1})=p_j^\pi$.
	\qed
%\end{proof}
%
%\paragraph{Hardness of the gap problem}
%We now prove that the vector of probabilities
%$(\sqrt{W},\sqrt{W})$, if feasible, is isolated

	The following lemma is the last step of the reduction: if there is a strategy
	achieving a probability vector close to~$(\sqrt{W},\sqrt{W})$ by
	some~$\epsilon$, then there is a pure strategy achieving exactly
	$(\sqrt{W},\sqrt{W})$. The reduction follows.

			\begin{lemma}
				\label{lemma:hardness-epsilon}
				Given $v_1,\ldots,v_n \in \mathbb{Z}^+$, and $W = \prod_{i=1}^n
				\frac{1}{v_i}$, let $\epsilon < \frac{1}{4}\sqrt{W}$.
				%\frac{2W}{1+\sqrt{W}}$.
				If there exists a strategy~$\tau$ such that for~$i=1,2$, $p_i^\tau =  \sqrt{W}+\delta_i$
				for some $\delta_1,\delta_2 \in [-\epsilon,\epsilon]$, 
				then there is a pure strategy achieving probabilities $(\sqrt{W},\sqrt{W})$.
			\end{lemma}
			\begin{proof}
				Consider any~$\sigma$ with value vector~$(\sqrt{W}+\delta_1,\sqrt{W}+\delta_2)$.
				If we write $\sigma$ as the linear combination of pure strategies
				as $\sigma = \sum_{i=1}^n \lambda_i \pi_i$, we get
				\[
					\begin{array}{l}
						\lambda_1 w_1 + \ldots + \lambda_n w_n = \sqrt{W}+\delta_1,\\
						\lambda_1 W/w_1 + \ldots + \lambda_n W/w_n = \sqrt{W}+\delta_2,\\
					\end{array}
				\]
				where $w_i = p^{\pi_i}_1$, and $W/w_i = p^{\pi_i}_2$.
				By dividing the second equation by~$W$, and distributing the right hand side in
				the linear combination in both lines, we rewrite this as
				\[
					\begin{array}{l}
						\lambda_1 (w_1-\sqrt{W}) + \ldots + \lambda_n (w_n-\sqrt{W}) = \delta_1,\\
			%			\lambda_1 (\frac{w_1 - \sqrt{W} - \frac{w_1\delta_2}{\sqrt{W}}}{w_1\sqrt{W}}) + \ldots + \lambda_n
			%			(\frac{w_n-\sqrt{W}- \frac{w_n\delta_2}{\sqrt{W}}}{w_n\sqrt{W}}) = 0.\\
						\lambda_1 (\frac{w_1 - \sqrt{W}}{w_1\sqrt{W}}) + \ldots + \lambda_n
						(\frac{w_n-\sqrt{W}}{w_n\sqrt{W}}) - \frac{\delta_2}{W} = 0.\\
					\end{array}
				\]
				Towards a contradiction, assume that $w_i \neq \sqrt{W}$ for all~$i$.
			%	Let~$N' = N \cap \{ i \mid w_i \neq \sqrt{W}\}$ and define similarly $P'$.
				Define $P \subsetneq \{1,\ldots,n\}$, the set of~$i$
				such that $w_i - \sqrt{W}>0$, and let~$N = \{1,\ldots,n\} \setminus P$.
				For all~$i\in P$, we have $1/w_i \geq \sqrt{1/W}+1$ which means
				$w_i \geq \frac{\sqrt{W}}{1-\sqrt{W}}$. For~$i\in N$, we similarly obtain
				$w_i \leq \frac{\sqrt{W}}{1+\sqrt{W}}$.
				We obtain that for any $i \in P$, $\frac{1}{w_i\sqrt{W}} \leq \frac{1-\sqrt{W}}{W}$,
				and for any $i \in N$, $\frac{1}{w_i\sqrt{W}} \geq \frac{1+\sqrt{W}}{W}$.
				We rewrite
				\begin{equation}
					\label{eqn:NP}
					\begin{array}{l}
						\sum_{i \in P} \lambda_i (w_i - \sqrt{W}) - \sum_{i \in N} \lambda_i
						(\sqrt{W}-w_i) = \delta_1 \in [-\epsilon,\epsilon],\\
						\sum_{i \in P} \lambda_i \frac{w_i - \sqrt{W}}{w_i\sqrt{W}}
						+\frac{\delta_2}{W}\sum_{i \in P}\lambda_i = 
						\sum_{i \in N} \lambda_i \frac{\sqrt{W}-w_i}{w_i\sqrt{W}}
			-\frac{\delta_2}{W}\sum_{i \in N}\lambda_i.
					\end{array}
				\end{equation}
				We have
				\[
					\begin{array}{l}
						\frac{1+\sqrt{W}}{W}\sum_{i \in N}\lambda_i (\sqrt{W}-w_i) -
						\frac{\delta_2}{W}\sum_{i \in N} \lambda_i\\
						\leq \sum_{i \in N} \lambda_i \frac{\sqrt{W}-w_i}{w_i\sqrt{W}} -
						\frac{\delta_2}{W}\sum_{i \in N} \lambda_i\\
						=
						\sum_{i \in P} \lambda_i \frac{w_i - \sqrt{W}}{w_i\sqrt{W}} +
						\frac{\delta_2}{W}\sum_{i \in P} \lambda_i\\
						\leq \frac{1-\sqrt{W}}{W} \sum_{i \in P}\lambda_i (w_i - \sqrt{W}) + 
						\frac{\delta_2}{W}\sum_{i \in P} \lambda_i.\\
					\end{array}
				\]
				It folows that $(1+\sqrt{W})\alpha_N - (1-\sqrt{W})\alpha_P \leq \delta_2$,
				where~$\alpha_P = \sum_{i \in P}\lambda_i(w_i - \sqrt{W})$ and
				similarly for~$\alpha_N$.  We must have $(\alpha_N-\alpha_P) +
				\sqrt{W}(\alpha_N+\alpha_P) \leq \epsilon$.
				Because $\alpha_P-\alpha_N \in [-\epsilon,\epsilon]$, we have
				$\sqrt{W}(\alpha_N+\alpha_P) \leq 2\epsilon$.
				But we have that $|w_i -\sqrt{W}| \geq \frac{\sqrt{W}}{1+\sqrt{W}}$
				so $\alpha_N+\alpha_P\geq \frac{\sqrt{W}}{1+\sqrt{W}}$.
				It follows that $\frac{W}{1+\sqrt{W}} \leq 2\epsilon$, which is a
				contradiction.
			\end{proof}


\begin{proof}[of Lemma~\ref{lemma:gaphard}]
%	Assume there is a procedure~$\calP$ for the~$\epsilon$-gap problem in MEMDPs.
%	We prove that $\calP$ can be used to solve the \textsf{Subset-Product} problem.
	We reduce \textsf{Subset-Product} to the $\epsilon$-gap problem for
	reachability in MEMDPs.
	Consider an instance given by $v_1,\ldots,v_n, V$ and consider the MEMDP~$M$
	constructed above with starting state~$s_1$ and target~$\{s_n\}$.
	Let~$W$ and~$\epsilon$ be given by the above lemma. 

	If \textsf{Subset-Product} has a solution, then there exists a pure strategy
	in~$M$ achieving $(\sqrt{W},\sqrt{W})$ and the~$\epsilon$-gap instance is
	positive. If there is \textsf{Subset-Product} has no solution, then there is
	no pure strategy achieving this vector. Therefore, by
	Lemma~\ref{lemma:hardness-epsilon}, there is no
	strategy achieving at least $(\sqrt{W}-\epsilon,\sqrt{W}-\epsilon)$
	componentwise. Thus, the $\epsilon$-gap instance is negative.
\end{proof}


\iffalse
				We will now show that any strategy that achieves $(\sqrt{W},\sqrt{W})$ is a
				linear combination of pure strategies with the same value vector.

				%For any path~$\pi$ (or deterministic strategy) we let
				%$w_\pi = p^\pi_1 (  =\prod_{i \in S_\pi} v_i^{-1})$.
				%We know that $p^\pi_2 = W/w_\pi$. 
				Consider any~$\sigma$ with value
				vector~$(\sqrt{W},\sqrt{W})$.
				If we write $\sigma$ as the linear combination of pure strategies
				as $\sigma = \sum_{i=1}^n \lambda_i \pi_i$, we get
				\[
					\begin{array}{l}
						\lambda_1 w_1 + \ldots + \lambda_n w_n = \sqrt{W},\\
						\lambda_1 W/w_1 + \ldots + \lambda_n W/w_n = \sqrt{W},\\
					\end{array}
				\]
				where $w_i = p^{\pi_i}_1$, and $W/w_i = p^{\pi_i}_2$.
				By dividing the second equation by~$W$, and distributing the right hand side in
				the linear combination in both lines, we rewrite this as
				\[
					\begin{array}{l}
						\lambda_1 (w_1-\sqrt{W}) + \ldots + \lambda_n (w_n-\sqrt{W}) = 0,\\
						\lambda_1 (\frac{w_1 - \sqrt{W}}{w_1\sqrt{W}}) + \ldots + \lambda_n
						(\frac{w_n-\sqrt{W}}{w_n\sqrt{W}}) = 0.\\
					\end{array}
				\]
				Towards a contradiction, assume that there exists~$i$ such that $w_i \neq
				\sqrt{W}$. Define $\emptyset \neq P \subsetneq \{1,\ldots,n\}$, the set of~$i$
				such that $w_i - \sqrt{W}>0$, and let~$N = \{1,\ldots,n\} \setminus P$.
				Observe that for any $i \in P$, $\frac{1}{w_n\sqrt{W}} < \frac{1}{W}$,
				and for any $i \in N$, $\frac{1}{w_n\sqrt{W}} \geq \frac{1}{W}$.
				We have 
				\begin{equation}
					\label{eqn:NP}
					\begin{array}{l}
						\sum_{i \in P} \lambda_i (w_i - \sqrt{W}) = \sum_{i \in N} \lambda_i
						(\sqrt{W}-w_i),\\
						\sum_{i \in P} \lambda_i \frac{w_i - \sqrt{W}}{w_i\sqrt{W}} = 
						\sum_{i \in N} \lambda_i \frac{\sqrt{W}-w_i}{w_i\sqrt{W}},
					\end{array}
				\end{equation}
				and a similar equality can be written for the second equation.
				On the one hand, $\sum_{i \in P} \lambda_i (\frac{w_i - \sqrt{W}}{w_i\sqrt{W}}) 
				< \frac{1}{W} \sum_{i \in P} \lambda_i (w_i - \sqrt{W})$. On the other hand,
				$\frac{1}{W} \sum_{i \in P} \lambda_i (w_i - \sqrt{W})=\frac{1}{W} \sum_{i \in N} \lambda_i (\sqrt{W}- w_i) \leq \sum_{i \in N}
				\lambda_i (\frac{\sqrt{W} - w_i}{w_i\sqrt{W}}) $
				which contradicts the second line of \eqref{eqn:NP}.

				\medskip
				The theorem follows.
\fi


==> safety.tex <==
\section{Safety Objectives}
\label{section:safety}
Recall that almost-sure and sure safety coincide in MEMDPs.
The equivalence of almost-sure and sure safety with limit-sure safety is less
trivial, and follows from Lemma~\ref{lemma:only11-inf}:
%It follows from Lemma~\ref{lemma:only11-inf} that limit-sure and almost-sure safety
%objectives coincide in MEMDPs.
\begin{lemma}
	Limit-sure safety is equivalent to almost-sure safety in MEMDPs.
\end{lemma}

The following lemma shows how sure safety objectives can be solved in polynomial time.
\footnote{This lemma gives a direct characterization of winning states for sure
safety objectives. Note however that the almost-sure parity algorithm can be
used to decide sure safety. (This remark does not hold for reachability since
the parity algorithm uses reachability as a subprocedure).
Should we remove this lemma?
}


